LHC and B physics probes of neutrinoless double beta decay in supersymmetry without R-parity

In the event of an observation of neutrinoless double beta decay, a relevant question would be: what lepton number violating physics is responsible for the decay? The exchange of Majorana neutrinos and/or supersymmetric particles may contribute. We point out that measurements of supersymmetric signals at the LHC, including single slepton production, could be used to help bound some supersymmetric processes contributing to neutrinoless double beta decay. LHC information about the supersymmetric spectrum could be combined with Bd-Bd bar mixing data in order to bound a competing neutrinoless double beta decay process involving sbottom exchange.

==> preamble.tex <==
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
%DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

